A geometric reformulation of the bilevel parameter optimization problem to a single level non-linear programming problem with applications to phase equilibria

Phase equilibrium problems are central to chemical engineering, underpinning tasks ranging from separation process design to the development of thermodynamic models. A particularly challenging computational task is the generation of phase envelopes: rigorously fitting thermodynamic models to real world data with well behaved predictions requires solving a computationally expensive bilevel optimization problem. We present a geometric reformulation of this parameter estimation problem that restates the bilevel program as a single level problem that is significantly easier to solve. The solution of the single level problem is proven to be the globally optimal solution of the bilevel problem when specialized global optimization solvers are used. In addition, the method retains the constraints that guarantee a well behaved fitted model, such as enforcing the correct number of phase splits, excluding spurious phases, and ensuring stability in regions of instability. This allows the practitioner to reliably and efficiently fit mathematically complex thermodynamic models to data, and potentially enables highly accurate and rigorous modelling of problems in computational thermodynamics that were previously intractable. Finally, an algorithm is presented that is proven to converge for any black box thermodynamic model. Only an expression of the Gibbs free energy is required, no derivatives are needed, and convergence is guaranteed for the broadest class of non-smooth, non-continuous models.

==> sections/supp_ccs_refrig_per_point.tex <==
% !TEX root = ../supplementary_S3_ccs_refrig.tex
% ------------------------------------------------------------------
% Supplementary Material S3 body: per-tie-line Gibbs / dual-manifold
% archives for the CCS quaternary and refrigerant R-407C cases (main
% manuscript, CCS and refrigerant results sections). Figure blocks are
% generated by the plot.py of figures/appendix-ccs-ternary/ and
% figures/appendix-refrig-ternary/ from raw data produced by
% scripts_ccs_manuscript_figdata.py / scripts_refrig_manuscript_figdata.py
% at the fitted parameters.
% ------------------------------------------------------------------

Analogously to the sour-gas archive of Supplementary Material~S2,
this supplement records the
reduced Gibbs energy and dual manifold along every model tie-line
section of the two remaining industrial validation sets, evaluated at
the respective fitted parameters $\mathbf{p}^{\star}$ with the section
construction defined there. Both records are fully defect-free:
$\mathcal{M} \geq 0$ holds along every section with equality only at
the two phase compositions.

\subsection{CCS quaternary: CO$_2$/Ar/O$_2$ validation tie lines}
\label{supp:ccs-per-point}

The 18 ternary validation tie lines
of~\cite{CoqueletArpentinier2014} at the CO$_2$-$X$ parameters
reported in the CCS results section of the main manuscript, with air
pairs ideal ($k_{a,ij}=0$).

\input{figures/appendix-ccs-ternary/appendix-ccs-ternary_figure_blocks}

\clearpage
\subsection{Refrigerant R-407C: ternary validation tie lines}
\label{supp:refrig-per-point}

The 44 ternary validation tie lines of~\cite{KatoNishiumi2006} at
the binary-fitted parameters reported in the refrigerant results
section of the main manuscript.

\input{figures/appendix-refrig-ternary/appendix-refrig-ternary_figure_blocks}


==> sections/supp_sour_gas_per_point.tex <==
% !TEX root = ../supplementary_S2_sour_gas.tex
% ------------------------------------------------------------------
% Supplementary Material S2 body: per-tie-line Gibbs / dual-manifold
% archive for the sour-gas ternary case (main manuscript, sour-gas
% results section). The 31 figure blocks are generated by
% figures/appendix-sour-gas-ternary/plot.py (which also emits
% figure_blocks.tex) from raw data produced by
% scripts_sour_gas_manuscript_figdata.py at the fitted parameters.
% ------------------------------------------------------------------

In this supplement we archive, for every one of the 31 experimental
ternary tie lines of Theveneau et al.~\cite{Theveneau2020}
% [PDF: page 3, Table 2 and page 4, Table 3] - the 31 validation tie lines
used to validate the sour-gas case of the main manuscript,
the reduced Gibbs energy and the dual manifold evaluated at the fitted
parameters $\mathbf{p}^{\star}$. Because the equilibrium here is
vapor--liquid at elevated pressure, the one-dimensional section shown
for each tie line is taken along the \emph{model} tie line: the
segment $\mathbf{x}(s) = (1-s)\,\mathbf{x}^{\mathrm{exp}}_{\mathrm{I}}
+ s\,\mathbf{y}^{\mathrm{mod}}$, $s \in [-0.05, 1.05]$, joining the
experimental liquid composition to the vapor composition returned by
the bubble-point calculation at $(T_i, p^{\mathrm{mod}}_i)$. For each
tie line the left panel shows the minimum-root reduced Gibbs energy
$g(\mathbf{x}(s), \mathbf{p}^{\star})$ together with the
common-tangent chord $h$ between the two phase compositions; the
right panel shows the dual manifold
$\mathcal{M}(\mathbf{x}(s); \mathbf{p}^{\star}) = g - h$, whose
negative part $[\mathcal{M}]_{-}$ enters the bilevel objective. A
defect-free solution requires $\mathcal{M} \geq 0$ along the entire
section, with equality only at the two phase compositions. The plots
below constitute the point-by-point record of that property for the
regressed sour-gas parameters: 27 of the 31 sections are defect-free
to numerical tolerance, while the four highest-pressure near-critical
tie lines (18, 19, 24 and 27; $p = 13.6$--$15.4$~MPa) show shallow
negative lobes of magnitude
$\lvert \min \mathcal{M} \rvert \leq 2.5 \times 10^{-5}$, visible in
the corresponding manifold panels and discussed in the sour-gas
results section of the main manuscript.

\input{figures/appendix-sour-gas-ternary/appendix-sour-gas-ternary_figure_blocks}

